TRAVERSE: Traffic-Responsive Autonomous Vehicle Experience & Rare-event Simulation for Enhanced safety

Data for training learning-enabled self-driving cars in the physical world are typically collected in a safe, normal environment. Such data distribution often engenders a strong bias towards safe driving, making self-driving cars unprepared when encountering adversarial scenarios like unexpected accidents. Due to a dearth of such adverse data that is unrealistic for drivers to collect, autonomous vehicles can perform poorly when experiencing such rare events. This work addresses much-needed research by having participants drive a VR vehicle simulator going through simulated traffic with various types of accidental scenarios. It aims to understand human responses and behaviors in simulated accidents, contributing to our understanding of driving dynamics and safety. The simulation framework adopts a robust traffic simulation and is rendered using the Unity Game Engine. Furthermore, the simulation framework is built with portable, light-weight immersive driving simulator hardware, lowering the resource barrier for studies in autonomous driving research. Keywords: Rare Events, Traffic Simulation, Autonomous Driving, Virtual Reality, User Studies

==> sections/features.tex <==
\section{\textbf{Simulator Features}}

\subsection{\textbf{Interactive Traffic Simulation}}
The traffic simulations conducted in SUMO enabled our study to craft a highly interactive environment that was responsible for vehicle movements, accidents, and animal crossing. This aided the study in augmenting immersion and realism while driving the simulator.


\subsection{\textbf{Customizable scenario creation}}
Vast models of road layout can be implemented successfully in Roadrunner. This facilitated our study by letting us build road models designed for a particular scenario.


\subsection{\textbf{Server connectivity}}
To enhance the realism of driving scenarios, an additional controller setup can be introduced to govern the behavior of the accident-inducing vehicle. This extension involves establishing a client-server architecture within the game engine, enabling data transmission from a secondary computer to the host system. Control over the secondary vehicle can be facilitated through various input methods such as keyboards, controllers, or an additional steering wheel configuration. Alternatively, even a single-computer setup allows for concurrent control of both the primary and secondary vehicles using distinct steering wheel setups or keyboard inputs.

\subsection{\textbf{Integrating Eye Gaze, head pose, and hand tracking}}
To integrate eye-gaze, head, and hand-tracking functionalities, the Meta Quest Pro VR device is selected for its advantageous blend of affordability and user-friendliness relative to other available alternatives. Leveraging both the Meta-XR Core SDK and Movement SDK, the system adeptly tracks and records pertinent data, including eye gaze and head pose, facilitating subsequent post-analysis. Additionally, through the implementation of hand interaction via the Movement SDK, users experience heightened immersion, as they can seamlessly control steering using their hands.
 
\subsection{\textbf{ROS Compatibility}}
The simulator seamlessly integrates with both ROS1 and ROS2 through the utilization of the ROS-TCP protocol package provided within the game engine. This compatibility ensures that users can leverage the simulator within the broader ROS ecosystem, facilitating the development, testing, and deployment of robotic systems across different ROS versions with ease.

\subsection{\textbf{Weather Conditions, Day/Dawn/Night}}

To augment the robustness of the data collected during the study, fundamental environmental factors like rain and different times of day were altered. Distinct weather conditions can greatly affect the quality of perception and hence, it is necessary to include them in the dataset.

\subsection{\textbf{Side view, Rear View Mirrors, Headlights, Brakelights and Indicator}}

To enhance realism, the simulator includes side and rearview mirrors with cameras for simulated reflections. Functional brake lights, turn signals, and headlights are also implemented. Brake lights illuminate when braking, turn signals flash for lane changes, and headlights adjust based on the environment, like turning on at night. These features enhance visual fidelity and create an immersive driving experience.

\subsection{\textbf{Ambient Environmental sounds}}
Every sound-inducing factor in traffic including engine revving, skidding, and horns was included in the simulator. C\# scripts coded to generate sound were included in UNITY to augment the user experience driving.


\subsection{\textbf{Unlimited assets available}}
A wealth of assets can be integrated with this driving simulator, including a diverse selection of vehicles, realistic human models, and a variety of animals and birds. These assets are readily accessible from popular stores like the Unity Asset Store and animation platforms like Mixamo. Incorporating these assets into our driving simulator is a seamless process, enhancing the simulation's realism and immersive experience.


==> sections/method.tex <==
\section{Methodology}

%\subsection{Creating Scenarios}

The main motivation is to craft diverse and challenging accident-inducing situations for simulation, inspired by NHTSA pre-crash typology, to capture data showing how human drivers respond to adversaries and their spontaneity to make the ideal decisions leading to the least impact. An impactful feature of the study involves a randomized sequence of the 8 scenarios for each driver, consequently preventing user bias. The duration of each scenario lasts approximately 45 to 60 seconds, a sufficient window to facilitate a thorough evaluation of their reaction time under different accident scenarios.\\

The simulator integration architecture involves importing 3D static scenes from Roadrunner and incorporating simulated traffic scenarios from the traffic simulator into the game engine. The latter plays a vital role in visualizing and interacting with the scenarios with complete immersion. Additionally, it may also function as a user interface for communicating and monitoring autonomous driving systems during simulation.\\

Every scenario includes traffic cars, controlled through the traffic simulator. Communication between the game engine and traffic simulator is established using the Coding Connected TraCI Net, which is an open-source C\# library based on the Python framework. A client/server is instantiated in a port of the system to establish connectivity between the game engine and the traffic simulator. 

% The number of vehicles in the simulation is determined at each time step and traffic car positions are adjusted accordingly. The traffic lights operate in phases, cycling again upon completion of all phases. 
% The initiation and termination of the scenarios are executed using the buttons on the keyboard.\\

\begin{figure}[htp]
    \centering
    \includegraphics[width=8cm]{images/software_integration.jpg}
    \caption{Softwares..}
    \label{fig:galaxy}
\end{figure}

Accident scenarios such as Jaywalking pedestrian, (including deer) vehicle lane change without indication can be simulated and used for future autonomous driving research purposes. These scenarios collectively offer a robust framework for evaluating and enhancing the safety of autonomous driving in a mixed autonomy where real drivers and self-driving agents co-exist, providing valuable insights into their decision-making, collision avoidance, and adaptability in diverse and challenging real-world situations.

% Eight driving scenarios, each designed to simulate specific challenging situations for autonomous vehicles have been developed, along with an additional practice scenario for initial familiarization with the environment and hardware. These scenarios encompass a diverse range of potential hazards, providing a comprehensive testbed for assessing the performance and decision-making abilities of autonomous driving systems.
% Practice Scenario: 
% Purpose: To familiarize the system and users with the simulation environment. 
% Description: This scenario involves basic driving tasks in a controlled setting without any traffic cars, allowing users to get accustomed to the simulator and vehicle controls.

% Sudden Lane Change without Indication: 
% Purpose: Assessing the system's response to abrupt lane changes without turn signal indication. 
% Description: The vehicle encounters a sudden lane change scenario, requiring adaptive decision-making to navigate safely while respecting traffic rules.

% T-Bone Crash: 
% Purpose: Evaluating collision avoidance capabilities during a T-bone collision scenario. 
% Description: Simulates a T-bone crash situation, challenging the system to react promptly and take appropriate actions to prevent or mitigate the impact.

% Sudden Stop: 
% Purpose: Testing the system's ability to respond to an unexpected stop without proper signaling. 
% Description: The vehicle confronts an abrupt stop scenario, demanding quick and precise reactions to avoid collisions while signaling appropriately.

% Running Red Light: 
% Purpose: Evaluating adherence to traffic signals and assessing stopping decisions after violating a red light. 
% Description: The vehicle runs a red light and is then required to stop, assessing the system's ability to correct course after a rule violation. 

% Deer Crossing: 
% Purpose: Assessing the system's capability to detect and respond to unexpected obstacles, in this case, a deer crossing the road. 
% Description: Simulates a scenario where a deer suddenly crosses the road, challenging the system to identify and navigate around the obstacle safely.

% Crash in Roundabout: 
% Purpose: Testing navigation and collision avoidance in a complex roundabout environment. 
% Description: The vehicle navigates a roundabout, encountering a simulated crash scenario, and assessing the system's ability to make informed decisions in a complex traffic environment. 

% Sudden Merge from Ramp: 
% Purpose: Evaluating merging capabilities and response to unexpected accidents during lane changes. 
% Description: Simulates a scenario where an accident occurs while the vehicle is merging lanes, challenging the system to navigate and respond effectively.

% Pedestrian Crossing: 
% Purpose: Assessing the system's capability to detect and respond to unexpected obstacles, in this case, a pedestrian crossing the road.
% Description: Simulates a scenario where a pedestrian suddenly crosses the road, challenging the system to identify and navigate around the obstacle safely.







==> sections/simulator.tex <==
\section{Driving Simulator}
\subsection{Software}
\subsubsection{\textbf{Scene Creation}}

RoadRunner by MathWorks is a tool for creating detailed and realistic 3D scenes with complex road networks and landscapes. It offers a user-friendly interface for designing road layouts, terrain features, and structures. Users can also utilize Open Street Map (OSM) to provide real-world geographical data, but OSM falls short in customization capabilities, lacking options for detailed features such as lanes, traffic signals, and signboards.

RoadRunner addresses these limitations by allowing users to create region-specific road signs and markings, and insert various 3D models enabling highly customized roadway scenes. It offers three Levels of Detail (LOD) for road network models, balancing performance and visual fidelity. Additionally, RoadRunner supports importing and exporting road networks in formats like FBX for game engines and OpenDrive for traffic simulators, streamlining the workflow for developers to create and transfer scenarios to other platforms seamlessly.

\subsubsection{\textbf{Traffic Simulation}}

SUMO (Simulation of Urban MObility) enhances driving scenario realism by modeling vehicle movement, traffic flow, and intersections. SUMO complements RoadRunner by providing a microscopic simulation of continuous, multimodal vehicle traffic in large urban road networks. Its advanced features, like lane-changing behaviors and traffic light control, enhance simulated traffic dynamics, facilitating the exploration of complex driving scenarios. Additionally, SUMO's Floating Car Data (FCD) feature provides precise information for every vehicle in the network, including location and speed at each time step, enriching the evaluation process.

\subsubsection{\textbf{Physics Engine}}

To convert the 2D traffic simulation to 3D, Unity, a popular game development engine is employed to integrate the road maps created in RoadRunner along with the dynamic 2D traffic scenarios simulated by the traffic simulator. Unity provides a powerful platform for creating immersive simulations, and its compatibility with various modeling and simulation tools makes it an ideal choice for merging different components.

\subsection{Hardware}

\subsubsection{\textbf{Virtual Reality}}

To enhance user immersion, the integration of a VR device has been implemented. The Meta Quest Pro has been selected especially for its eye-gaze tracking functionality for post-simulation research. In instances where eye-tracking data is deemed unnecessary for the intended research purposes, any other VR alternatives such as Quest 1 or Quest 2 can be utilized.

\subsubsection{\textbf{Steering Wheel}}

In order to enhance the fidelity and realism of the driving simulation, the Logitech G29 steering wheel, coupled with its pedal kit, has been meticulously chosen as the input device that enables precise control over the vehicle, surpassing the limitations of conventional keyboard or controller inputs. This setup offers inputs for acceleration, braking, steering, and gear shifting (Drive and Reverse). These input signals are seamlessly integrated with Unity, facilitating accurate and immersive control over the ego vehicle within the driving simulation environment.
 
\subsubsection{\textbf{PC Specifications}}
This simulator has been developed in the Windows 11 x64 system. Other specifications are as follows: Processor: Intel Xenon(R) Gold 5218 CPU (x2 Processor), RAM: 64GB, Graphics: Nvidia GeForce RTX 2080 Ti and Storage: 2TB SSD.

The cost of the total hardware setup including Meta VR, Steering Wheel, and the PC is \$.... approximately.

\subsection{Integration}

The simulator integration architecture involves importing 3D static scenes from Roadrunner and incorporating simulated traffic scenarios from the traffic simulator into the game engine. The latter plays a vital role in visualizing and interacting with the scenarios with complete immersion. Additionally, it may also function as a user interface for communicating and monitoring autonomous driving systems during simulation. Communication between the game engine and traffic simulator is established using the Coding Connected TraCI Net, which is an open-source C\# library based on the Python framework. A client/server is instantiated in a port of the system to establish connectivity between the game engine and the traffic simulator. 

==> sections/tables/pvalue.tex <==
\begin{table}[!ht]
\centering
\caption{\small{Comparison of various criteria between two VR driving simulators. The table presents t-statistics, p-values, and indicates whether there is a significant difference between the simulators in each criterion}}
\begin{tabular}{|p{3.5cm}|p{1.25cm}|p{1cm}|p{1.5cm}|}
\hline
\textbf{Comparison Criterion} & \textbf{t statistic} & \textbf{p-value} & \textbf{Significant \newline Difference \newline (Yes/No)} \\ \hline
Sense of Being in VR          & 3.895                & 0.000249         & Yes                                       \\ 
Ease of adjustment   & 5.748                & 3.22e-07        & Yes                                       \\ 
Scenario Realism             & 3.164                & 0.002445         & Yes                                       \\
Controls Responsiveness       & 4.476                & 3.41e-05        & Yes                                       \\ 
Audio Immersiveness              & 2.046                & 0.045190         & Yes                                       \\ 
Head Tracking                & 4.801                & 1.08e-05        & Yes                                       \\
Traffic Simulation            & 0.620                & 0.537284         & No                                        \\
Real-world Driving Accuracy   & 4.238                & 7.89e-05        & Yes                                       \\
Overall Experience            & 5.595                & 5.76e-07        & Yes                                       \\  \hline
\end{tabular}
\label{tb:T-Test}

\end{table}


==> sections/tables/qual_comparison_table.tex <==
\begin{table}[t!]
  \centering
  \scalebox{.70}{
  \begin{tabular}{lccccccc}
    % \toprule
   Method & \phantom{a} & \rot{Pre-crash Simulation} & \rot{Virtual Reality} & \rot{Human Interaction} & \rot{Traffic Simulation} & \rot{Open Source} \\
    \midrule
    DrEyeVR & \phantom{a} & \xmark  & \cmark & \cmark & \xmark & \cmark \\
    Ours & \phantom{a} & \cmark  & \cmark & \cmark & \cmark & \cmark\\
    \bottomrule
  \end{tabular}}
%   \vspace*{-0.25em}
 \caption{
Qualitative comparison between our simulator and existing simulators for autonomous driving data collection and user studies. 
}
\vspace{-1.5em}
  \label{tb:qual_comparison}
\end{table}

